ActiveRMAP: Radiance Field for Active Mapping And Planning

A high-quality 3D reconstruction of a scene from a collection of 2D images can be achieved through offline/online mapping methods. In this paper, we explore active mapping from the perspective of implicit representations, which have recently produced compelling results in a variety of applications. One of the most popular implicit representations - Neural Radiance Field (NeRF), first demonstrated photorealistic rendering results using multi-layer perceptrons, with promising offline 3D reconstruction as a by-product of the radiance field. More recently, researchers also applied this implicit representation for online reconstruction and localization (i.e. implicit SLAM systems). However, the study on using implicit representation for active vision tasks is still very limited. In this paper, we are particularly interested in applying the neural radiance field for active mapping and planning problems, which are closely coupled tasks in an active system. We, for the first time, present an RGB-only active vision framework using radiance field representation for active 3D reconstruction and planning in an online manner. Specifically, we formulate this joint task as an iterative dual-stage optimization problem, where we alternatively optimize for the radiance field representation and path planning. Experimental results suggest that the proposed method achieves competitive results compared to other offline methods and outperforms active reconstruction methods using NeRFs.

==> content/problem.tex <==
\section{Problem statement}
We consider two active vision problems in this paper (active 3D reconstruction and active navigation). 
% 
\textbf{Active 3D reconstruction}: a robot is tasked with autonomously reconstructing a scene or object of interest.
% 
\textbf{Active navigation}: a robot is tasked with navigating to a goal destination, given the destination robot states (\eg 6-DoF camera pose). 
% 
We make three assumptions about the robotic agent. 
(1) it is equipped with a RGB camera;
(2) it is capable of localizing itself within the environment;
and (3) an accurate kinematic module that allows it to move precisely to a given state.


==> fig_tab_alg/alg_active_nav.tex <==


% \begin{center}
\begin{algorithm} 
    \caption{Active Visual Navigation}
  \begin{algorithmic}[1]
    \INPUT DVGO coarse model $\textbf{M}^{(c)}$; goal state $\textbf{s}_g$
    \STATE \textbf{Initialization} agent state $s_t=s_{0}$; image database $\{I\}_{i=0}^{0}$; STOP=False
    \STATE \textbf{Coarse Stage: }
        \Indent
        \WHILE{not STOP}
            \STATE \textbf{Local policy}: $\textbf{S}^* \leftarrow$  path planning (\cref{sec:method:planning})
            \STATE \textbf{Action}: $\textbf{s}_{t+1} \leftarrow \textbf{s}^*$ 
                % \Comment{move to the next feasible state $\textbf{s}^*$. }
            \STATE \textbf{Observation}: obtain a new image observation $I_t$
            \STATE \textbf{Update database}: $\{I\}_{i=0}^{t+1} \leftarrow \{I\}_{i=0}^{t}$
            \STATE \textbf{Optimize DVGO}: $\textbf{M}^{(c)}_{t+1} \leftarrow \textbf{M}^{(c)}_t$ 
            % \Comment{optimize the DVGO coarse model based on the database up-to-date \cref{sec:dvgo}} 
            % \STATE \textbf{Update Entropy Volume}: update $\textbf{V}^{(E,c)}$
            \STATE \textbf{Check STOP}: check STOP condition
        \ENDWHILE
        \EndIndent
  \end{algorithmic}
\label{alg:active_recon}
\end{algorithm} 
% \end{center}


==> fig_tab_alg/tab_geometry_result.tex <==
% 
\begin{table} [th!]  
    \begin{center}
    \resizebox{1\columnwidth}{!}{%
    \begin{tabular}{ l |  c  c c | c c c } 
        % \hline
        % \cline{2-9}
        Methods &
        PSNR $\uparrow$ & 
        SSIM $\uparrow$ & 
        LPIPS $\downarrow$ & 
        PSNR $\uparrow$ & 
        SSIM $\uparrow$ & 
        LPIPS $\downarrow$ \\
        \hline
        \hline
        & \multicolumn{6}{c}{\textbf{Synthetic-NeRF}}  \\
         & \multicolumn{3}{c | }{Discrete (local), 10 views}  & \multicolumn{3}{c}{Discrete (local), 20 views}  \\ 
        \hline
        Random &
        16.869	& 0.789	 & 0.215 &
        20.435	& 0.839	 & 0.160 \\

        FVS & 
        18.683 &	0.805 &	0.189 &
        23.470 &	0.872 &	0.127 \\

        \textbf{Entropy} &
        \textbf{19.358} &	\textbf{0.820} &	\textbf{0.172} &
        \textbf{23.936} & 	\textbf{0.880} &	\textbf{0.118} \\
        \hline
        \hline

        %%%%%%%%%%%%%%%%%%%%%%%%
         & \multicolumn{3}{c | }{Discrete (free), 10 views}  & \multicolumn{3}{c}{Discrete (free), 20 views}  \\ 
        \hline
        ActiveNeRF \cite{pan2022activenerf} &
        20.010 & 0.832 & 0.204 &
        \textbf{26.240}  & 0.856 & 0.124 \\
        
        % Random &
        % 21.208 &	0.839 &	0.151 &
        % \textbf{25.249} &	\textbf{0.894} &	\textbf{0.105} \\

        \textbf{Entropy} &
        \textbf{21.853} &	\textbf{0.846} &	\textbf{0.144} &
        24.489 &	\textbf{0.888} &	\textbf{0.113} \\
        \hline
        \hline

        \multicolumn{7}{}{} \\

        \multicolumn{7}{c}{\textbf{Tanks \& Temples (Discrete (local), 50 views)}}  \\
        & 
        \multicolumn{2}{c}{PSNR $\uparrow$} & 
        \multicolumn{2}{c}{SSIM $\uparrow$} & 
        \multicolumn{2}{c}{LPIPS $\downarrow$} \\
        \hline
        \hline
        % \multicolumn{7}{c}{Discrete (local), 50 views}    \\ 

        % \hline
        Random &
        \multicolumn{2}{c}{18.169} & 
        \multicolumn{2}{c}{0.827} & 
        \multicolumn{2}{c}{0.225} \\
        % 18.169 & 	0.827	 & 0.2246 \\

        FVS & 
        \multicolumn{2}{c}{20.240} & 
        \multicolumn{2}{c}{0.844} & 
        \multicolumn{2}{c}{0.204} \\
        % 18.683 &	0.805 &	0.189 &
        % 20.240 &	0.844 &	0.204 \\

        \textbf{Entropy} &
        \multicolumn{2}{c}{\textbf{21.560}} & 
        \multicolumn{2}{c}{\textbf{0.848}} & 
        \multicolumn{2}{c}{\textbf{0.200}} \\
        \hline
        % 19.358 &	0.820 &	0.172 &
        % 21.560 &	0.848 &	0.200 \\
        % \hline
        % \hline

        %         Random &
        % 16.869	& 0.789	 & 0.215 &
        % 18.169 & 	0.827	 & 0.2246 \\

        % FVS & 
        % 18.683 &	0.805 &	0.189 &
        % 20.240 &	0.844 &	0.204 \\

        % Entropy &
        % 19.358 &	0.820 &	0.172 &
        % 21.560 &	0.848 &	0.200 \\
    \end{tabular}
    }
    \end{center}
    % \vspace{-1em}
    \caption{
        Next best view policy comparison (Geometry). 
        ``\textbf{Discrete (local), N views}" means the camera is limited to local motion and the view space is limited to the discrete viewpoints in the training set. Up to N views can be used for training.
        ``\textbf{Discrete (free)}" means teleporting between viewpoints in the training set is allowed.   
    }
    \label{table:exp:rendering_result}
    % \vspace{-25pt}
\end{table}
% % 
